Catalogue of Phonon Instabilities in Symmetry Group 191 Kagome MT$_6$Z$_6$ Materials

Kagome materials manifest rich physical properties due to the emergence of abundant electronic phases. Here, we carry out a high-throughput first-principles study of the kagome 1:6:6 family MT$_6$Z$_6$ materials in space group 191, focusing on their phonon instability and electronic flat bands. Different MT$_6$Z$_6$ kagome candidates reveal a remarkable variety of kagome flat bands ranging from unfilled, partially filled, to fully filled. Notably, the Mn/Fe-166 compounds exhibit partially filled flat bands with a pronounced sharp peak in the density of states near the Fermi level, leading to magnetic orders that polarize the bands and stabilize the otherwise unstable phonon. When the flat bands are located away from the Fermi level, we find a large number of phonon instabilities, which can be classified into three types, based on the phonon dispersion and vibrational modes. Type-I instabilities involve the in-plane distortion of kagome nets, while type-II and type-III present out-of-plane distortion of trigonal M and Z atoms. We take MgNi$_6$Ge$_6$ and HfNi$_6$In$_6$ as examples to illustrate the possible CDW structures derived from the emergent type-I and type-II instabilities. The type-I instability in MgNi$_6$Ge$_6$ suggests a nematic phase transition, governed by the local twisting of kagome nets. The type-II instability in HfNi$_6$In$_6$ may result in a hexagonal-to-orthorhombic transition, offering insight into the formation of MT$_6$Z$_6$ in other space groups. Additionally, the predicted ScNb$_6$Sn$_6$ is analyzed as an example of the type-III instability. Our predictions suggest a vast kagome family with rich properties induced by the flat bands, possible CDW transitions, and their interplay with magnetism.

==> table/stat09_3.tex <==
\begin{table}[htbp]
\global\long\def\arraystretch{1.12}
\captionsetup{width=.95\textwidth}
\caption{Brief collection of phonon results for \ch{MT6Z6} compounds. HLS denotes stable phonon at both low-T and high-T, HSLU denotes stable phonon at high-T but unstable phonon at low-T, and HLU denotes unstable phonon at both high-T and low-T. Here, the finite temperature phonon are calculated at harmonic level via smearing approach. High-T and low-T denote a Fermi-Dirac smearing value of 0.4 eV and 0.05 eV, respectively.}
\label{Tab:SM_phononcollection}
\setlength{\tabcolsep}{1.mm}{
\begin{tabular}{c|c|l|c|l}
\hline
\hline
 & Count & Materials & Count & Materials  \\
\hline
HLS & 6 & \parbox{1.2cm}{VSn, VGe, CrGe, CoSn, NiIn, NbSn} & 166 & \parbox{12cm}{$M$V$_6$Ge$_6$($M$=\hyperref[sms2sec:LiV6Ge6]{{\color{green} Li }}, \hyperref[sms2sec:ScV6Ge6]{{\color{green} Sc }}, \hyperref[sms2sec:TiV6Ge6]{{\color{green} Ti }}, \hyperref[sms2sec:YV6Ge6]{{\color{green} Y }}, \hyperref[sms2sec:ZrV6Ge6]{{\color{green} Zr }}, \hyperref[sms2sec:NbV6Ge6]{{\color{green} Nb }}, \hyperref[sms2sec:PrV6Ge6]{{\color{green} Pr }}, \hyperref[sms2sec:NdV6Ge6]{{\color{green} Nd }}, \hyperref[sms2sec:SmV6Ge6]{{\color{green} Sm }}, \hyperref[sms2sec:GdV6Ge6]{{\color{green} Gd }}, \hyperref[sms2sec:TbV6Ge6]{{\color{green} Tb }}, \hyperref[sms2sec:DyV6Ge6]{{\color{green} Dy }}, \hyperref[sms2sec:HoV6Ge6]{{\color{green} Ho }}, \hyperref[sms2sec:ErV6Ge6]{{\color{green} Er }}, \hyperref[sms2sec:TmV6Ge6]{{\color{green} Tm }}, \hyperref[sms2sec:YbV6Ge6]{{\color{green} Yb }}, \hyperref[sms2sec:LuV6Ge6]{{\color{green} Lu }}, \hyperref[sms2sec:HfV6Ge6]{{\color{green} Hf }}, \hyperref[sms2sec:TaV6Ge6]{{\color{green} Ta }}), $M$V$_6$Sn$_6$($M$=\hyperref[sms2sec:LiV6Sn6]{{\color{green} Li }}, \hyperref[sms2sec:TiV6Sn6]{{\color{green} Ti }}, \hyperref[sms2sec:YV6Sn6]{{\color{green} Y }}, \hyperref[sms2sec:ZrV6Sn6]{{\color{green} Zr }}, \hyperref[sms2sec:NbV6Sn6]{{\color{green} Nb }}, \hyperref[sms2sec:PrV6Sn6]{{\color{green} Pr }}, \hyperref[sms2sec:NdV6Sn6]{{\color{green} Nd }}, \hyperref[sms2sec:SmV6Sn6]{{\color{green} Sm }}, \hyperref[sms2sec:GdV6Sn6]{{\color{green} Gd }}, \hyperref[sms2sec:TbV6Sn6]{{\color{green} Tb }}, \hyperref[sms2sec:DyV6Sn6]{{\color{green} Dy }}, \hyperref[sms2sec:HoV6Sn6]{{\color{green} Ho }}, \hyperref[sms2sec:ErV6Sn6]{{\color{green} Er }}, \hyperref[sms2sec:TmV6Sn6]{{\color{green} Tm }}, \hyperref[sms2sec:LuV6Sn6]{{\color{green} Lu }}, \hyperref[sms2sec:HfV6Sn6]{{\color{green} Hf }}, \hyperref[sms2sec:TaV6Sn6]{{\color{green} Ta }}), $M$Cr$_6$Ge$_6$($M$=\hyperref[sms2sec:LiCr6Ge6]{{\color{green} Li }}, \hyperref[sms2sec:MgCr6Ge6]{{\color{green} Mg }}, \hyperref[sms2sec:CaCr6Ge6]{{\color{green} Ca }}, \hyperref[sms2sec:ScCr6Ge6]{{\color{green} Sc }}, \hyperref[sms2sec:TiCr6Ge6]{{\color{green} Ti }}, \hyperref[sms2sec:YCr6Ge6]{{\color{green} Y }}, \hyperref[sms2sec:ZrCr6Ge6]{{\color{green} Zr }}, \hyperref[sms2sec:NbCr6Ge6]{{\color{green} Nb }}, \hyperref[sms2sec:PrCr6Ge6]{{\color{green} Pr }}, \hyperref[sms2sec:NdCr6Ge6]{{\color{green} Nd }}, \hyperref[sms2sec:SmCr6Ge6]{{\color{green} Sm }}, \hyperref[sms2sec:GdCr6Ge6]{{\color{green} Gd }}, \hyperref[sms2sec:TbCr6Ge6]{{\color{green} Tb }}, \hyperref[sms2sec:DyCr6Ge6]{{\color{green} Dy }}, \hyperref[sms2sec:HoCr6Ge6]{{\color{green} Ho }}, \hyperref[sms2sec:ErCr6Ge6]{{\color{green} Er }}, \hyperref[sms2sec:TmCr6Ge6]{{\color{green} Tm }}, \hyperref[sms2sec:YbCr6Ge6]{{\color{green} Yb }}, \hyperref[sms2sec:LuCr6Ge6]{{\color{green} Lu }}, \hyperref[sms2sec:HfCr6Ge6]{{\color{green} Hf }}, \hyperref[sms2sec:TaCr6Ge6]{{\color{green} Ta }}), $M$Mn$_6$Ge$_6$($M$=\hyperref[sms2sec:ScMn6Ge6]{{\color{green} Sc }}, \hyperref[sms2sec:TiMn6Ge6]{{\color{green} Ti }}, \hyperref[sms2sec:YMn6Ge6]{{\color{green} Y }}, \hyperref[sms2sec:ZrMn6Ge6]{{\color{green} Zr }}, \hyperref[sms2sec:NbMn6Ge6]{{\color{green} Nb }}, \hyperref[sms2sec:PrMn6Ge6]{{\color{green} Pr }}, \hyperref[sms2sec:NdMn6Ge6]{{\color{green} Nd }}, \hyperref[sms2sec:SmMn6Ge6]{{\color{green} Sm }}, \hyperref[sms2sec:GdMn6Ge6]{{\color{green} Gd }}, \hyperref[sms2sec:TbMn6Ge6]{{\color{green} Tb }}, \hyperref[sms2sec:DyMn6Ge6]{{\color{green} Dy }}, \hyperref[sms2sec:HoMn6Ge6]{{\color{green} Ho }}, \hyperref[sms2sec:ErMn6Ge6]{{\color{green} Er }}, \hyperref[sms2sec:TmMn6Ge6]{{\color{green} Tm }}, \hyperref[sms2sec:LuMn6Ge6]{{\color{green} Lu }}, \hyperref[sms2sec:HfMn6Ge6]{{\color{green} Hf }}, \hyperref[sms2sec:TaMn6Ge6]{{\color{green} Ta }}), $M$Co$_6$Sn$_6$($M$=\hyperref[sms2sec:LiCo6Sn6]{{\color{green} Li }}, \hyperref[sms2sec:MgCo6Sn6]{{\color{green} Mg }}, \hyperref[sms2sec:CaCo6Sn6]{{\color{green} Ca }}, \hyperref[sms2sec:ScCo6Sn6]{{\color{green} Sc }}, \hyperref[sms2sec:TiCo6Sn6]{{\color{green} Ti }}, \hyperref[sms2sec:YCo6Sn6]{{\color{green} Y }}, \hyperref[sms2sec:ZrCo6Sn6]{{\color{green} Zr }}, \hyperref[sms2sec:NbCo6Sn6]{{\color{green} Nb }}, \hyperref[sms2sec:PrCo6Sn6]{{\color{green} Pr }}, \hyperref[sms2sec:NdCo6Sn6]{{\color{green} Nd }}, \hyperref[sms2sec:SmCo6Sn6]{{\color{green} Sm }}, \hyperref[sms2sec:GdCo6Sn6]{{\color{green} Gd }}, \hyperref[sms2sec:TbCo6Sn6]{{\color{green} Tb }}, \hyperref[sms2sec:DyCo6Sn6]{{\color{green} Dy }}, \hyperref[sms2sec:HoCo6Sn6]{{\color{green} Ho }}, \hyperref[sms2sec:ErCo6Sn6]{{\color{green} Er }}, \hyperref[sms2sec:TmCo6Sn6]{{\color{green} Tm }}, \hyperref[sms2sec:YbCo6Sn6]{{\color{green} Yb }}, \hyperref[sms2sec:LuCo6Sn6]{{\color{green} Lu }}, \hyperref[sms2sec:HfCo6Sn6]{{\color{green} Hf }}, \hyperref[sms2sec:TaCo6Sn6]{{\color{green} Ta }}, \hyperref[sms2sec:TlCo6Sn6]{{\color{green} Tl }}), $M$Ni$_6$Si$_6$($M$=\hyperref[sms2sec:YNi6Si6]{{\color{green} Y }}, \hyperref[sms2sec:ZrNi6Si6]{{\color{green} Zr }}, \hyperref[sms2sec:PrNi6Si6]{{\color{green} Pr }}, \hyperref[sms2sec:NdNi6Si6]{{\color{green} Nd }}, \hyperref[sms2sec:SmNi6Si6]{{\color{green} Sm }}, \hyperref[sms2sec:GdNi6Si6]{{\color{green} Gd }}, \hyperref[sms2sec:TbNi6Si6]{{\color{green} Tb }}, \hyperref[sms2sec:DyNi6Si6]{{\color{green} Dy }}, \hyperref[sms2sec:HoNi6Si6]{{\color{green} Ho }}, \hyperref[sms2sec:ErNi6Si6]{{\color{green} Er }}), $M$Ni$_6$Ge$_6$($M$=\hyperref[sms2sec:CaNi6Ge6]{{\color{green} Ca }}, \hyperref[sms2sec:YNi6Ge6]{{\color{green} Y }}, \hyperref[sms2sec:ZrNi6Ge6]{{\color{green} Zr }}, \hyperref[sms2sec:PrNi6Ge6]{{\color{green} Pr }}, \hyperref[sms2sec:NdNi6Ge6]{{\color{green} Nd }}, \hyperref[sms2sec:SmNi6Ge6]{{\color{green} Sm }}, \hyperref[sms2sec:GdNi6Ge6]{{\color{green} Gd }}, \hyperref[sms2sec:TbNi6Ge6]{{\color{green} Tb }}, \hyperref[sms2sec:DyNi6Ge6]{{\color{green} Dy }}, \hyperref[sms2sec:HoNi6Ge6]{{\color{green} Ho }}, \hyperref[sms2sec:ErNi6Ge6]{{\color{green} Er }}, \hyperref[sms2sec:TmNi6Ge6]{{\color{green} Tm }}, \hyperref[sms2sec:YbNi6Ge6]{{\color{green} Yb }}, \hyperref[sms2sec:LuNi6Ge6]{{\color{green} Lu }}), $M$Ni$_6$In$_6$($M$=\hyperref[sms2sec:LiNi6In6]{{\color{green} Li }}, \hyperref[sms2sec:CaNi6In6]{{\color{green} Ca }}, \hyperref[sms2sec:ScNi6In6]{{\color{green} Sc }}, \hyperref[sms2sec:YNi6In6]{{\color{green} Y }}, \hyperref[sms2sec:ZrNi6In6]{{\color{green} Zr }}, \hyperref[sms2sec:NbNi6In6]{{\color{green} Nb }}, \hyperref[sms2sec:PrNi6In6]{{\color{green} Pr }}, \hyperref[sms2sec:NdNi6In6]{{\color{green} Nd }}, \hyperref[sms2sec:SmNi6In6]{{\color{green} Sm }}, \hyperref[sms2sec:GdNi6In6]{{\color{green} Gd }}, \hyperref[sms2sec:TbNi6In6]{{\color{green} Tb }}, \hyperref[sms2sec:DyNi6In6]{{\color{green} Dy }}, \hyperref[sms2sec:HoNi6In6]{{\color{green} Ho }}, \hyperref[sms2sec:ErNi6In6]{{\color{green} Er }}, \hyperref[sms2sec:YbNi6In6]{{\color{green} Yb }}), $M$Ni$_6$Sn$_6$($M$=\hyperref[sms2sec:LiNi6Sn6]{{\color{green} Li }}, \hyperref[sms2sec:MgNi6Sn6]{{\color{green} Mg }}, \hyperref[sms2sec:CaNi6Sn6]{{\color{green} Ca }}, \hyperref[sms2sec:ScNi6Sn6]{{\color{green} Sc }}, \hyperref[sms2sec:TiNi6Sn6]{{\color{green} Ti }}, \hyperref[sms2sec:YNi6Sn6]{{\color{green} Y }}, \hyperref[sms2sec:ZrNi6Sn6]{{\color{green} Zr }}, \hyperref[sms2sec:NbNi6Sn6]{{\color{green} Nb }}, \hyperref[sms2sec:PrNi6Sn6]{{\color{green} Pr }}, \hyperref[sms2sec:NdNi6Sn6]{{\color{green} Nd }}, \hyperref[sms2sec:SmNi6Sn6]{{\color{green} Sm }}, \hyperref[sms2sec:GdNi6Sn6]{{\color{green} Gd }}, \hyperref[sms2sec:TbNi6Sn6]{{\color{green} Tb }}, \hyperref[sms2sec:DyNi6Sn6]{{\color{green} Dy }}, \hyperref[sms2sec:HoNi6Sn6]{{\color{green} Ho }}, \hyperref[sms2sec:ErNi6Sn6]{{\color{green} Er }}, \hyperref[sms2sec:TmNi6Sn6]{{\color{green} Tm }}, \hyperref[sms2sec:YbNi6Sn6]{{\color{green} Yb }}, \hyperref[sms2sec:LuNi6Sn6]{{\color{green} Lu }}, \hyperref[sms2sec:HfNi6Sn6]{{\color{green} Hf }}, \hyperref[sms2sec:TaNi6Sn6]{{\color{green} Ta }}), $M$Nb$_6$Sn$_6$($M$=\hyperref[sms2sec:TiNb6Sn6]{{\color{green} Ti }}, \hyperref[sms2sec:YNb6Sn6]{{\color{green} Y }}, \hyperref[sms2sec:ZrNb6Sn6]{{\color{green} Zr }}, \hyperref[sms2sec:PrNb6Sn6]{{\color{green} Pr }}, \hyperref[sms2sec:NdNb6Sn6]{{\color{green} Nd }}, \hyperref[sms2sec:SmNb6Sn6]{{\color{green} Sm }}, \hyperref[sms2sec:GdNb6Sn6]{{\color{green} Gd }}, \hyperref[sms2sec:TbNb6Sn6]{{\color{green} Tb }}, \hyperref[sms2sec:DyNb6Sn6]{{\color{green} Dy }}, \hyperref[sms2sec:HfNb6Sn6]{{\color{green} Hf }})} \\ 
\hline
HSLU & 5 & \parbox{1.2cm}{MnSn, MnGe, FeGe, FeSn, CoGe} & 103 & \parbox{12cm}{\hyperref[sms2sec:CaV6Ge6]{{\color{blue} CaV$_6$Ge$_6$ }}, $M$V$_6$Sn$_6$($M$=\hyperref[sms2sec:CaV6Sn6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScV6Sn6]{{\color{blue} Sc }}, \hyperref[sms2sec:YbV6Sn6]{{\color{blue} Yb }}), $M$Mn$_6$Ge$_6$($M$=\hyperref[sms2sec:LiMn6Ge6]{{\color{blue} Li }}, \hyperref[sms2sec:MgMn6Ge6]{{\color{blue} Mg }}, \hyperref[sms2sec:CaMn6Ge6]{{\color{blue} Ca }}, \hyperref[sms2sec:YbMn6Ge6]{{\color{blue} Yb }}), $M$Mn$_6$Sn$_6$($M$=\hyperref[sms2sec:LiMn6Sn6]{{\color{blue} Li }}, \hyperref[sms2sec:MgMn6Sn6]{{\color{blue} Mg }}, \hyperref[sms2sec:CaMn6Sn6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScMn6Sn6]{{\color{blue} Sc }}, \hyperref[sms2sec:TiMn6Sn6]{{\color{blue} Ti }}, \hyperref[sms2sec:YMn6Sn6]{{\color{blue} Y }}, \hyperref[sms2sec:ZrMn6Sn6]{{\color{blue} Zr }}, \hyperref[sms2sec:NbMn6Sn6]{{\color{blue} Nb }}, \hyperref[sms2sec:PrMn6Sn6]{{\color{blue} Pr }}, \hyperref[sms2sec:NdMn6Sn6]{{\color{blue} Nd }}, \hyperref[sms2sec:SmMn6Sn6]{{\color{blue} Sm }}, \hyperref[sms2sec:GdMn6Sn6]{{\color{blue} Gd }}, \hyperref[sms2sec:TbMn6Sn6]{{\color{blue} Tb }}, \hyperref[sms2sec:DyMn6Sn6]{{\color{blue} Dy }}, \hyperref[sms2sec:HoMn6Sn6]{{\color{blue} Ho }}, \hyperref[sms2sec:ErMn6Sn6]{{\color{blue} Er }}, \hyperref[sms2sec:TmMn6Sn6]{{\color{blue} Tm }}, \hyperref[sms2sec:YbMn6Sn6]{{\color{blue} Yb }}, \hyperref[sms2sec:LuMn6Sn6]{{\color{blue} Lu }}, \hyperref[sms2sec:HfMn6Sn6]{{\color{blue} Hf }}, \hyperref[sms2sec:TaMn6Sn6]{{\color{blue} Ta }}), $M$Fe$_6$Ge$_6$($M$=\hyperref[sms2sec:LiFe6Ge6]{{\color{blue} Li }}, \hyperref[sms2sec:MgFe6Ge6]{{\color{blue} Mg }}, \hyperref[sms2sec:CaFe6Ge6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScFe6Ge6]{{\color{blue} Sc }}, \hyperref[sms2sec:TiFe6Ge6]{{\color{blue} Ti }}, \hyperref[sms2sec:YFe6Ge6]{{\color{blue} Y }}, \hyperref[sms2sec:ZrFe6Ge6]{{\color{blue} Zr }}, \hyperref[sms2sec:NbFe6Ge6]{{\color{blue} Nb }}, \hyperref[sms2sec:PrFe6Ge6]{{\color{blue} Pr }}, \hyperref[sms2sec:NdFe6Ge6]{{\color{blue} Nd }}, \hyperref[sms2sec:SmFe6Ge6]{{\color{blue} Sm }}, \hyperref[sms2sec:GdFe6Ge6]{{\color{blue} Gd }}, \hyperref[sms2sec:TbFe6Ge6]{{\color{blue} Tb }}, \hyperref[sms2sec:DyFe6Ge6]{{\color{blue} Dy }}, \hyperref[sms2sec:HoFe6Ge6]{{\color{blue} Ho }}, \hyperref[sms2sec:ErFe6Ge6]{{\color{blue} Er }}, \hyperref[sms2sec:TmFe6Ge6]{{\color{blue} Tm }}, \hyperref[sms2sec:YbFe6Ge6]{{\color{blue} Yb }}, \hyperref[sms2sec:LuFe6Ge6]{{\color{blue} Lu }}, \hyperref[sms2sec:HfFe6Ge6]{{\color{blue} Hf }}, \hyperref[sms2sec:TaFe6Ge6]{{\color{blue} Ta }}, \hyperref[sms2sec:UFe6Ge6]{{\color{blue} U }}), $M$Fe$_6$Sn$_6$($M$=\hyperref[sms2sec:LiFe6Sn6]{{\color{blue} Li }}, \hyperref[sms2sec:MgFe6Sn6]{{\color{blue} Mg }}, \hyperref[sms2sec:CaFe6Sn6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScFe6Sn6]{{\color{blue} Sc }}, \hyperref[sms2sec:TiFe6Sn6]{{\color{blue} Ti }}, \hyperref[sms2sec:YFe6Sn6]{{\color{blue} Y }}, \hyperref[sms2sec:ZrFe6Sn6]{{\color{blue} Zr }}, \hyperref[sms2sec:NbFe6Sn6]{{\color{blue} Nb }}, \hyperref[sms2sec:PrFe6Sn6]{{\color{blue} Pr }}, \hyperref[sms2sec:NdFe6Sn6]{{\color{blue} Nd }}, \hyperref[sms2sec:SmFe6Sn6]{{\color{blue} Sm }}, \hyperref[sms2sec:GdFe6Sn6]{{\color{blue} Gd }}, \hyperref[sms2sec:TbFe6Sn6]{{\color{blue} Tb }}, \hyperref[sms2sec:DyFe6Sn6]{{\color{blue} Dy }}, \hyperref[sms2sec:HoFe6Sn6]{{\color{blue} Ho }}, \hyperref[sms2sec:ErFe6Sn6]{{\color{blue} Er }}, \hyperref[sms2sec:TmFe6Sn6]{{\color{blue} Tm }}, \hyperref[sms2sec:YbFe6Sn6]{{\color{blue} Yb }}, \hyperref[sms2sec:LuFe6Sn6]{{\color{blue} Lu }}, \hyperref[sms2sec:HfFe6Sn6]{{\color{blue} Hf }}, \hyperref[sms2sec:TaFe6Sn6]{{\color{blue} Ta }}), $M$Co$_6$Ge$_6$($M$=\hyperref[sms2sec:LiCo6Ge6]{{\color{blue} Li }}, \hyperref[sms2sec:CaCo6Ge6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScCo6Ge6]{{\color{blue} Sc }}, \hyperref[sms2sec:TiCo6Ge6]{{\color{blue} Ti }}, \hyperref[sms2sec:YCo6Ge6]{{\color{blue} Y }}, \hyperref[sms2sec:ZrCo6Ge6]{{\color{blue} Zr }}, \hyperref[sms2sec:NbCo6Ge6]{{\color{blue} Nb }}, \hyperref[sms2sec:PrCo6Ge6]{{\color{blue} Pr }}, \hyperref[sms2sec:NdCo6Ge6]{{\color{blue} Nd }}, \hyperref[sms2sec:SmCo6Ge6]{{\color{blue} Sm }}, \hyperref[sms2sec:GdCo6Ge6]{{\color{blue} Gd }}, \hyperref[sms2sec:TbCo6Ge6]{{\color{blue} Tb }}, \hyperref[sms2sec:DyCo6Ge6]{{\color{blue} Dy }}, \hyperref[sms2sec:HoCo6Ge6]{{\color{blue} Ho }}, \hyperref[sms2sec:ErCo6Ge6]{{\color{blue} Er }}, \hyperref[sms2sec:TmCo6Ge6]{{\color{blue} Tm }}, \hyperref[sms2sec:YbCo6Ge6]{{\color{blue} Yb }}, \hyperref[sms2sec:LuCo6Ge6]{{\color{blue} Lu }}), $M$Ni$_6$Si$_6$($M$=\hyperref[sms2sec:CaNi6Si6]{{\color{blue} Ca }}, \hyperref[sms2sec:YbNi6Si6]{{\color{blue} Yb }}), $M$Ni$_6$In$_6$($M$=\hyperref[sms2sec:TiNi6In6]{{\color{blue} Ti }}, \hyperref[sms2sec:TmNi6In6]{{\color{blue} Tm }}, \hyperref[sms2sec:LuNi6In6]{{\color{blue} Lu }}, \hyperref[sms2sec:HfNi6In6]{{\color{blue} Hf }}, \hyperref[sms2sec:TaNi6In6]{{\color{blue} Ta }}), $M$Nb$_6$Sn$_6$($M$=\hyperref[sms2sec:CaNb6Sn6]{{\color{blue} Ca }}, \hyperref[sms2sec:ScNb6Sn6]{{\color{blue} Sc }}, \hyperref[sms2sec:HoNb6Sn6]{{\color{blue} Ho }}, \hyperref[sms2sec:ErNb6Sn6]{{\color{blue} Er }}, \hyperref[sms2sec:TmNb6Sn6]{{\color{blue} Tm }}, \hyperref[sms2sec:YbNb6Sn6]{{\color{blue} Yb }})} \\ 
\hline
HLU & 3 & \parbox{1.2cm}{NiGe, NiSi, NiSn} & 24 & \parbox{12cm}{\hyperref[sms2sec:MgV6Ge6]{{\color{red} MgV$_6$Ge$_6$ }}, \hyperref[sms2sec:MgV6Sn6]{{\color{red} MgV$_6$Sn$_6$ }}, $M$Co$_6$Ge$_6$($M$=\hyperref[sms2sec:MgCo6Ge6]{{\color{red} Mg }}, \hyperref[sms2sec:HfCo6Ge6]{{\color{red} Hf }}, \hyperref[sms2sec:TaCo6Ge6]{{\color{red} Ta }}, \hyperref[sms2sec:UCo6Ge6]{{\color{red} U }}), $M$Ni$_6$Si$_6$($M$=\hyperref[sms2sec:LiNi6Si6]{{\color{red} Li }}, \hyperref[sms2sec:MgNi6Si6]{{\color{red} Mg }}, \hyperref[sms2sec:ScNi6Si6]{{\color{red} Sc }}, \hyperref[sms2sec:TiNi6Si6]{{\color{red} Ti }}, \hyperref[sms2sec:NbNi6Si6]{{\color{red} Nb }}, \hyperref[sms2sec:LuNi6Si6]{{\color{red} Lu }}, \hyperref[sms2sec:HfNi6Si6]{{\color{red} Hf }}, \hyperref[sms2sec:TaNi6Si6]{{\color{red} Ta }}), $M$Ni$_6$Ge$_6$($M$=\hyperref[sms2sec:LiNi6Ge6]{{\color{red} Li }}, \hyperref[sms2sec:MgNi6Ge6]{{\color{red} Mg }}, \hyperref[sms2sec:ScNi6Ge6]{{\color{red} Sc }}, \hyperref[sms2sec:TiNi6Ge6]{{\color{red} Ti }}, \hyperref[sms2sec:NbNi6Ge6]{{\color{red} Nb }}, \hyperref[sms2sec:HfNi6Ge6]{{\color{red} Hf }}, \hyperref[sms2sec:TaNi6Ge6]{{\color{red} Ta }}), \hyperref[sms2sec:MgNi6In6]{{\color{red} MgNi$_6$In$_6$ }}, $M$Nb$_6$Sn$_6$($M$=\hyperref[sms2sec:LiNb6Sn6]{{\color{red} Li }}, \hyperref[sms2sec:MgNb6Sn6]{{\color{red} Mg }})} \\ 
\hline
\hline
\end{tabular}}
\end{table}


==> table/tab_phonon.tex <==
\begin{table*}[htbp]
\global\long\def\arraystretch{1.12}
% \captionsetup{width=.95\textwidth}
\caption{Collection of phonon stability with irreps for \ch{MT6Z6} kagome family, obtained by non-spin-polarized calculations without SOC. The first column denotes the $TZ$ ingredient, and the second column denotes the results for the CoSn-type $TZ$ structures, while the columns present the results for \ch{MT6Z6}. IRREPs denote the irreducible representations of the lowest imaginary phonon at high-symmetry points. "S" denotes the stable phonon at low-T. "-" are not included in this survey. "*" denote that they have been experimentally observed in either \ch{HfFe6Ge6}- or \ch{YCo6Ge6}-type hexagonal structure. Here, the finite temperature is considered at the harmonic level via the smearing approach. High-T and low-T refer to a Fermi-Dirac smearing of 0.4 eV and 0.05 eV, respectively. Red (blue) color denotes the unstable (stable) phonon at high-T. Note that in NiIn-166 the lowest modes obtained from $2\times2\times2$ supercells could be located at generic $\bm{q}$ instead of high-symmetry points, such as \ch{HfNi6In6} and \ch{LuNi6In6}. {Experimentally, instabilities have been reported in \ch{ScV6Sn6}~\cite{ScVSn2022}, \ch{MgCo6Ge6}~\cite{MgCoGe2021}, and \ch{YbCo6Ge6}~\cite{YbCoGe2022}.} The specific phonon spectra and notations are described in the Supplementary Note IV~\cite{supp}.}
\label{Tab:phonon}
\setlength{\tabcolsep}{0.6mm}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\hline
 & TZ & Li & Mg & Ca & Sc & Y & Lu & Ti & Zr & Hf & Nb & Ta & Pr & Nd & Sm & Gd & Tb & Dy & Ho & Er & Tm & Yb & U  \\
\hline
VGe & S & S & {\color{red}${H_4}$} & {\color{blue}${H_4}$} & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & -  \\ 
VSn & S & S & {\color{red}${H_4}$} & {\color{blue}${H_4}$} & {\color{blue}${H_4}$$^*$} & S$^*$ & S$^*$ & S & S & S & S & S & S & S & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & {\color{blue}${H_1}$$^*$} & -  \\ 
NbSn & S & {\color{red}${A_5^-}$} & {\color{red}${H_4}$} & {\color{blue}${H_4}$} & {\color{blue}${H_4}$} & S$^*$ & -  & S & S & S & -  & -  & S & S & S & S & S$^*$ & S & {\color{blue}${H_4}$} & {\color{blue}${H_4}$} & {\color{blue}${H_4}$} & {\color{blue}${H_4}$} & -  \\ 
CrGe & S & S & S & S & S$^*$ & S$^*$ & S & S & S & S & S & S & S & S & S & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & -  \\ 
MnGe & {\color{blue}${\Gamma_5^-}$} & {\color{blue}${\Gamma_5^-}$} & {\color{blue}${\Gamma_5^-}$$^*$} & {\color{blue}${\Gamma_5^-}$} & S$^*$ & S$^*$ & S$^*$ & S & S$^*$ & S$^*$ & S & S & S & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & {\color{blue}${\Gamma_5^-}$$^*$} & -  \\ 
MnSn & {\color{blue}${\Gamma_5^-}$} & {\color{blue}${\Gamma_5^-}$$^*$} & {\color{blue}${\Gamma_5^-}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_3^+}$$^*$} & {\color{blue}${\Gamma_5^-}$$^*$} & -  \\ 
FeGe & {\color{blue}${A_5^-}$}$^*$ & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_3^-}$$^*$} & {\color{blue}${A_3^-}$$^*$} & {\color{blue}${A_3^-}$$^*$} & {\color{blue}${\Gamma_3^-}$$^*$} & {\color{blue}${\Gamma_3^-}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_4^+}$$^*$} \\ 
FeSn & {\color{blue}${A_5^-}$}$^*$ & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${\Gamma_3^+}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^-}$$^*$} & {\color{blue}${A_5^+}$$^*$} & {\color{blue}${A_5^+}$} & -  \\ 
CoGe & {\color{blue}${\Gamma_3^-}$} & {\color{blue}${A_3^-}$$^*$} & {\color{red}${A_3^-}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${A_4^+}$$^*$} & {\color{blue}${A_4^+}$$^*$} & {\color{red}${A_4^+}$$^*$} & {\color{blue}${A_3^-}$} & {\color{red}${A_3^-}$} & {\color{blue}${\Gamma_4^+}$} & {\color{blue}${\Gamma_4^+}$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$$^*$} & {\color{red}${A_4^+}$$^*$} \\ 
CoSn & S$^*$ & S & S & S & S & S$^*$ & S$^*$ & S & S & S & S & S & S & S & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S$^*$ & S & -  \\ 
NiSi & {\color{red}${A_2^-}$} & {\color{red}${A_3^-}$$^*$} & {\color{red}${\Gamma_4^+}$$^*$} & {\color{blue}${\Gamma_4^+}$} & {\color{red}${\Gamma_4^+}$} & S & {\color{red}${\Gamma_4^+}$} & {\color{red}${\Gamma_4^+}$} & S & {\color{red}${\Gamma_4^+}$} & {\color{red}${A_4^+}$} & {\color{red}${A_4^+}$} & S & S & S & S & S & S & S & S & S & {\color{blue}${\Gamma_4^+}$} & -  \\ 
NiGe & {\color{red}${A_2^-}$} & {\color{red}${A_3^-}$$^*$} & {\color{red}${\Gamma_4^+}$$^*$} & S & {\color{red}${\Gamma_4^+}$$^*$} & S & S & {\color{red}${\Gamma_4^+}$} & S & {\color{red}${\Gamma_4^+}$} & {\color{red}${A_3^-}$} & {\color{red}${A_3^-}$} & S & S & S & S & S & S & S & S & S & S & -  \\ 
NiSn & {\color{red}${A_2^-}$} & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & S & -  \\ 
NiIn & S$^*$ & S & {\color{red}${K_4}$} & S & S & S & {\color{blue}${M_3^-}$} & {\color{blue}${M_3^-}$} & S & {\color{blue}${M_3^-}$} & S & {\color{blue}${M_3^-}$} & S & S & S & S & S & S & S & S & {\color{blue}${M_3^-}$} & S & -  \\ 
\hline
\hline
\end{tabular}}
\end{table*}

==> table/table166.tex <==
% \begin{landscape}
% \begin{sidewaystable*}[ht]
\begin{table*}[ht]\label{tab:SM_struct1}
\global\long\def\arraystretch{1.1}
\caption{Brief collection of $MT_6Z_6$ reported in experiments or databases. $MT_6Z_6$ can crystallize in space groups 191 $P6/mmm$, 71 $Immm$, 65 $Cmmm$, 63 $Cmcm$, 62 $Pnma$. Typical structures can be found in Fig.~\ref{Fig:166}.}
\centering
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{rccccccc} 
  \hline
  \hline

M(TZ)$_6$ & VSn & VGe & CrGe & MnSn & MnGe & FeGa & FeGe \\
\hline
Li [$2s^1$]  & 191$^a$ & 65$^a$ &  & 191~\cite{LiMnSn2006,LiMnSn2021} &  &  & $^1$191~\cite{CoFeNiGe1981}   \\ 
\hline
Mg [$3s^2$]  & 191$^a$ & 191$^a$ &  & 191~\cite{MgZrHfMnSn2002} & {\color{black} 191}~\cite{MgMnGe2008} &  & $^1${\color{black} 191}~\cite{CoFeNiGe1981}  \\ 
Ca [$4s^2$]  &  &  &  & 191~\cite{MgCaMnSn1998} &  &  & $^{0.5}${\color{black} 191}~\cite{CaFeCoGe2023}, 63~\cite{CaFeGe2022,CaFeCoGe2023}   \\ 
\hline
Sc [$3d^1$] & $^1$191~\cite{ScVSn2022} & 191$^a$ & $^1${\color{black}191}~\cite{ScCrGe1988} & $^1${\color{black} 191}~\cite{RMnSn1991} & $^1${\color{black} 191}~\cite{RTGe1992,ZrLuScMnGe1999} & 71~\cite{RFeGa1990} & $^1${\color{black} 191}~\cite{RTGe1992}   \\ 
Y [$4d^1$] & $^1${\color{black}191}~\cite{RVSn2011,GdVSn2021,YVSnGdVSn2021} & 191$^a$ & $^1${\color{black}191}~\cite{YCrGe2013,YCrGe2022}  & $^1$191~\cite{RMnSn1991,YMnSn2021} & $^1$191~\cite{RTGe1992,YMnGe-LuMnSn1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RFeGe1994}, $^{0.76}$63~\cite{RTGe1992,RFeGe1994}  \\ 
Lu [$5d^1$] & $^{0.962}${\color{black}191}~\cite{RVSn2011} &  &  & $^1${\color{black} 191}~\cite{RMnSn1991,YMnGe-LuMnSn1993,RMnSn1999} & $^1${\color{black} 191}~\cite{RTGe1992,ZrLuScMnGe1999} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RTGe1992,YLuHfFeGe1998,RFeGeSn2001}   \\ 
\hline
Ti [$3d^2$] & 191$^a$ &  &  &  &  &  & $^1$191~\cite{ScTiZrHfNb2000}   \\ 
Zr [$4d^2$] & 191$^a$ &  &  & $^1$191~\cite{MgZrHfMnSn2002} & $^1${\color{black} 191}~\cite{ZrLuScMnGe1999} & 71~\cite{RFeGa1990} & $^1${\color{black} 191}~\cite{ScTiZrHfNb2000}    \\ 
Hf [$5d^2$] & 191$^a$ &  &  & $^1${\color{black} 191}~\cite{MgZrHfMnSn2002} & $^1${\color{black} 191}~\cite{HfMnGe2006} & 71~\cite{RFeGa1990} & $^1${\color{black} 191}~\cite{YLuHfFeGe1998,ScTiZrHfNb2000}   \\ 
\hline
Nb [$4d^4$] &  &  &  &  &  &  & $^1${\color{black} 191}~\cite{ScTiZrHfNb2000}  \\ 
\hline
\hline
Pr [$4f^3$] &  &  &  & 71~\cite{PrNdSmMnSn1993} &  &  &    \\ 
Nd [$4f^4$] &  &  &  & 71~\cite{PrNdSmMnSn1993} & $^{0.5}${\color{black} 191}~\cite{RTGe1992} &  &     \\ 
Sm [$4f^6$] & $^{0.78}${\color{black} 191}~\cite{SmVSn2023} &  &  & $^{0.75}${\color{black} 191}~\cite{RMnSnScFeSn1988,NdSmMnSn1997}, 71~\cite{PrNdSmMnSn1993} & $^{0.5}${\color{black} 191}~\cite{RTGe1992} & 71$^b$ & $^{0.5}${\color{black} 191}$^{c}$~\cite{salamakha1999ternary}   \\ 
Gd [$4f^75d^1$] & $^{0.932}${\color{black}191}~\cite{RVSn2011,GdVSn2021,YVSnGdVSn2021} &  & $^1$191~\cite{GdCrGe1993} & 191~\cite{RMnSn1991,GdMnSn2012,GdMnSn2020} & $^1$191~\cite{RTGe1992,RMnGe1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RFeGe1994,RFeGeSn2001}, 62~\cite{RTGe1992}    \\ 
Tb [$4f^9$] & 191~\cite{TbVSn2022,TbTmVSn2022} &  & $^{0.816}${\color{black} 191}~\cite{RCrGe1994} & $^1$191~\cite{RMnSn1991,RMnSn1999,TbMnSn2020} & $^{0.994}${\color{black}191}~\cite{RTGe1992,RMnGe1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RFeGe1994}, 63~\cite{RTGe1992,RFeGe1994}  \\ 
Dy [$4f^{10}$] & $^{0.914}${\color{black}191}~\cite{RVSn2011,TbTmVSn2022} &  & $^{0.916}${\color{black} 191}~\cite{DyHoErYCrGe1997} & 191~\cite{RMnSn1991} & $^1$191~\cite{RTGe1992,RMnGe1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$,63~\cite{RTGe1992,RFeGeSn2001}    \\ 
Ho [$4f^{11}$] & $^{0.936}${\color{black}191}~\cite{RVSn2011,GdHoVSn2021,TbTmVSn2022} &  & $^1${\color{black} 191}~\cite{DyHoErYCrGe1997}  & $^1$191~\cite{RMnSn1991,RMnSn1999} & $^1$191~\cite{RTGe1992,RMnGe1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$, 63~\cite{RTGe1992,RFeGeSn2001}   \\ 
Er [$4f^{12}$] & $^{0.893}${\color{black}191}~\cite{RVSn2011,TbTmVSn2022} &  & $^{0.958}${\color{black} 191}~\cite{DyHoErYCrGe1997}  & {\color{black} 191}~\cite{RMnSn1991,RMnSn1999} & $^{0.991}${\color{black}191}~\cite{RTGe1992,RMnGe1993} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$, 71~\cite{RTGe1992,RFeGe1994,RFeGeSn2001}    \\ 
Tm [$4f^{13}$] & $^{0.957}${\color{black}191}~\cite{RVSn2011,TbTmVSn2022} &  & 191~\cite{RCrGe2020} & $^{0.972}${\color{black}191}~\cite{RMnSn1991,RMnSn1999} & $^1${\color{black} 191}~\cite{RTGe1992} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$, 71~\cite{RTGe1992,RFeGeSn2001}   \\ 
Yb [$4f^{14}$] & 191~\cite{YbVSn2022} &  & 191~\cite{RCrGe2020,YbVSn2022} & $^{0.5}$191~\cite{YbMnSn1999} & $^{0.997}${\color{black}191}~\cite{RTGe1992} & 71~\cite{RFeGa1990} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RTGe1992,RFeGeSn2001}    \\ 
U [$5f^{3}6d^1$] &  &  &  &  &  & 71~\cite{UFeGa2006} & $^{0.5}${\color{black} 191}$^{c}$~\cite{UFeGe1994}    \\

\hline
\hline
\end{tabular}}
\begin{tablenotes}
\item $^a$ Structures obtained from Open Quantum Materials Database (OQMD)~\cite{OQMD2013};
\item $^b$ Structures obtained from Materials Project~\cite{MaterialsProject2013};
\item $^c$ occupation info obtained from ICSD, denoting the occupation of M atom at $1a(0,0,0)$ position. $0.5$ will lead to type-I disorder structure.
\end{tablenotes}
\label{tab:166_1}
\end{table*}

% \end{sidewaystable*}
% \end{landscape}




% \begin{landscape}
% \begin{sidewaystable*}[ht]
\begin{table*}[ht]\label{tab:SM_struct2}
\global\long\def\arraystretch{1.1}
\caption{Brief collection of MT$_6$Z$_6$ with space group info. Generally at room temperature, they can crystallize in space group 191 $P6/mmm$, 71 $Immm$, 65 $Cmmm$, 63 $Cmcm$, 62 $Pnma$.}
\centering
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{rcccccccc} 
  \hline
  \hline
M(TZ)$_6$ & FeSn & FeAl & CoGa & CoGe & CoSn & NiSi & NiGe & NbSn \\
\hline
Li [$2s^1$]  &  &  &  & $^1${\color{black} 191}~\cite{CoFeNiGe1981} & 191$^a$ & $^1$191~\cite{CoFeNiGe1981} & $^1$191~\cite{CoFeNiGe1981} &   \\ 
\hline
Mg [$3s^2$]  & 191$^a$ &  &  & $^1${\color{black} 191}~\cite{CoFeNiGe1981,MgCoGe2006,MgCoGe2021} & 65$^a$ & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} &   \\ 
Ca [$4s^2$]  &  &  &  & $^{0.5}${\color{black} 191}~\cite{CaFeCoGe2023}, 71~\cite{CaFeCoGe2023} &  &  &  &   \\ 
\hline
Sc [$3d^1$] & $^{0.85}${\color{black} 191}~\cite{RMnSnScFeSn1988} & 71$^b$ & 71$^b$ & $^1${\color{black} 191}~\cite{CoFeNiGe1981} & 65$^a$ & $^{0.5}${\color{black} 191}$^{c}$ & $^1$191~\cite{CoFeNiGe1981} &   \\ 
Y [$4d^1$] & $^{0.5}${\color{black} 191}$^{c}$, 71~\cite{RFeSn1991,RFeGeSn2001} & 71$^b$ & 71$^b$ & $^{0.5}${\color{black} 191}$^{c}$~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984,YCoSn2017} &  & 191$^a$ & $^1${\color{black} 191}~\cite{YNbSn2012}  \\ 
Lu [$5d^1$] & $^{0.5}${\color{black} 191}$^{c}$~\cite{RFeGeSn2001} &  &  & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} &  &  &   \\ 
\hline
Ti [$3d^2$] & 191$^a$ &  &  & $^1${\color{black} 191}~\cite{TiCoGe2019} & 65$^a$ &  & 191$^a$ &   \\ 
Zr [$4d^2$] & $^{0.75}${\color{black} 191}~\cite{ScTmLuZrFeSn2000} & 71$^b$ & 71$^b$ & $^1${\color{black} 191}~\cite{CoFeNiGe1981} & 191$^a$ &  & 191$^a$ &   \\ 
Hf [$5d^2$] & 191$^a$ & 71$^b$ &  & $^1${\color{black} 191}~\cite{CoFeNiGe1981} & 191$^a$ &  & 191$^a$ &   \\ 
\hline
Nb [$4d^4$] &  &  &  &  &  &  &  & $-$  \\ 
\hline
\hline
Pr [$4f^3$]  &  & 71$^b$ &  &  &  &  &  &   \\ 
Nd [$4f^4$] &  &  &  &  &  &  &  &   \\ 
Sm [$4f^6$] & $^{0.5}${\color{black} 191}~\cite{SmFeSn2000} &  &  & $^{0.5}${\color{black} 191}$^{c}$ & $^{0.5}${\color{black} 191}$^{c}$ &  &  &   \\ 
Gd [$4f^75d^1$] & $^{0.5}${\color{black} 191}$^{c}$, 63~\cite{RFeSn1991,RFeGeSn2001} & 71$^b$ &  & $^{0.5}${\color{black} 191}$^{c}$~\cite{CoFeNiGe1981} & $^{0.5}$ {\color{black} 191}$^{c}$ &  &  &   \\ 
Tb [$4f^9$] & $^{0.5}${\color{black} 191}$^{c}$, 63~\cite{RFeSn1991,RFeGeSn2001} & 71$^b$ & 71$^b$ & $^{0.5}${\color{black} 191}$^{c}$~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} & &  & $^1${\color{black} 191}~\cite{TbNbSn2010}  \\ 
Dy [$4f^{10}$] & $^{0.5}${\color{black} 191}$^{c}$,~65~\cite{RFeSn1991}, 63~\cite{RFeGeSn2001} & 71$^b$ & 71$^b$ & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} &  &  &   \\ 
Ho [$4f^{11}$] & $^{0.5}${\color{black} 191}$^{c}$, 71~\cite{RFeSn1991,RFeGeSn2001} & 71$^b$ & 71$^b$ & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} &  &  &   \\ 
Er [$4f^{12}$] & $^{0.5}${\color{black} 191}$^{c}$,63~\cite{RFeSn1991} & 71$^b$ & 71$^b$ & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} & & &   \\ 
Tm [$4f^{13}$] & $^{0.5}${\color{black} 191}$^{c}$~\cite{RFeGeSn2001} &  &  & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981} & $^{0.5}${\color{black} 191}$^{c}$~\cite{RCoSn1984} &  &  &   \\ 
Yb [$4f^{14}$] &  & 71$^b$ &  & $^{0.5}${\color{black} 191}~\cite{CoFeNiGe1981,YbCoGe2020,YbCoGe2022} &  &  &  &   \\ 
U [$5f^{3}6d^1$] &  & 71$^b$ &  & $^1$191~\cite{CoFeNiGe1981} &  &  &  &   \\
\hline
\hline
\end{tabular}}
\label{tab:166_2}
\end{table*}
% \end{sidewaystable*}
% \end{landscape}
